Behavioral Cloning via Search in Embedded Demonstration Dataset

Behavioural cloning uses a dataset of demonstrations to learn a behavioural policy. To overcome various learning and policy adaptation problems, we propose to use latent space to index a demonstration dataset, instantly access similar relevant experiences, and copy behavior from these situations. Actions from a selected similar situation can be performed by the agent until representations of the agent's current situation and the selected experience diverge in the latent space. Thus, we formulate our control problem as a search problem over a dataset of experts' demonstrations. We test our approach on BASALT MineRL-dataset in the latent representation of a Video PreTraining model. We compare our model to state-of-the-art Minecraft agents. Our approach can effectively recover meaningful demonstrations and show human-like behavior of an agent in the Minecraft environment in a wide variety of scenarios. Experimental results reveal that performance of our search-based approach is comparable to trained models, while allowing zero-shot task adaptation by changing the demonstration examples.

==> appendices_sep.tex <==



\maketitle


\begin{abstract}
Behavioural cloning uses a dataset of demonstrations to learn a behavioural policy. To overcome various learning and policy adaptation problems, we propose to use latent space to index a demonstration dataset, instantly access similar relevant experiences, and copy behavior from these situations. Actions from a selected similar situation can be performed by the agent until representations of the agent's current situation and the selected experience diverge in the latent space. Thus, we formulate our control problem as a search problem over a dataset of experts' demonstrations. We test our approach on BASALT MineRL-dataset in the latent representation of a Video PreTraining model. We compare our model to state-of-the-art Minecraft agents. Our approach can effectively recover meaningful demonstrations and show human-like behavior of an agent in the Minecraft environment in a wide variety of scenarios. Experimental results reveal that performance of our search-based approach is comparable to trained models, while allowing zero-shot task adaptation by changing the demonstration examples.

\end{abstract}

\section{Introduction}

\textit{Imitation Learning} (IL)~\cite{Schaal1996} and \textit{Reinforcement Learning} (RL)~\cite{SuttonBarto1998} are commonly used methods to train agents to perform tasks in simulated and real environments, including multi-skill agents. Despite the extensive research in these fields, there are persistent challenges that pose difficulties for IL and RL methods. Firstly, these methods typically require significant computational resources for training. Secondly, when faced with new experiences, retraining or fine-tuning of trained models becomes necessary. Thirdly, the lack of one-shot or few-shot adaptability is a bottleneck, which is current focus of numerous studies on large language \cite{ouyang2022training} and vision models \cite{oquab2023dinov2}. Exploring alternative approaches to IL and RL methods for control problems can potentially address these challenges and yield advantages in specific application domains.



A multi-modal latent space can be used for measuring similarity and multi-modal search. Some common ways to achieve multi-modal mapping is \textit{contrastive learning} \cite{radford2021learning} and \textit{supervised learning}, where in the later case representation at the last layers or a few layers before the output can serve as a multi-modal latent space \cite{baker2022video}. For control tasks, such multi-modal latent space can be used to connect visual and action experiences based on a demonstration dataset. Thus, database search in this latent space can provide actions for control. Such an approach can lead to improvements with respect to the three general challenges for IL and RL approaches mentioned above. 




\paragraph{Motivation}
The present study is motivated by the MineRL BASALT 2022 challenge \cite{ShahDragan2021, Milani2023}. In the challenge, an agent must solve the four tasks: find a cave, build an animal pen, build a village house, and make a waterfall~\cite{ShahDragan2021, Milani2023}. For these tasks, no reward function is provided. Agents were judged by human contractors on two criteria: success in the task and human-likeliness of behaviour. Although, the objective is not mathematically well-defined, for a human, the success in completing such tasks is easy to evaluate and select the best one out of two performance examples. To solve the tasks, participants had a dataset of expert demonstrations at their disposal. Each demonstration trajectory of image-action pairs contains a single episode of one of the tasks solved by a human expert. Simplest solution to this then is {\em behavioral cloning} (BC), where policy is trained using supervised learning. 

BC is limited by the expert demonstration trajectories used in the training, and due to the training scheme used, sampled action per state is optimal in terms of expectation. But in practice agents are facing different {\em situations} throughout the episode, where one might be avoiding an obstacle and other to search for suitable location. These situations each then clearly require different solutions. 

To this end, we introduce {\em search-based behavioural cloning} (S-BC), an approach to BC that addresses that issue. S-BC generates a latent space of experts' trajectories that encapsulate both present and past information, and reformulates the control problem as a search problem in such a space.  By allowing to search for {\em new} closest situation from the set of expert trajectories, our method in a effect {\em adapts} to the evaluation episode. 





\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\columnwidth]
    {figs/VPT-Architecture3.pdf}
    \caption{A scheme of the VPT model used in this study. An image input is encoded with an IMPALA CNN and passed through four transformer heads. Then, two MLP heads predict a keyboard and a mouse action respectively.}
    \label{fig:vpt_architecture}
    \vspace{-0.1in}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/example_search.pdf}
    \caption{An example of the search mechanism. At each timestep, we keep track of the distance between current and reference embedding. Whenever the distance overcomes a threshold, a divergence-based search (red line) selects a new reference embedding; if the agent follows a threshold for too long, a time-based search (blue line) is triggered.}
    \label{fig:divergence}
\end{figure}


\section{Related work}
BC has been successfully applied to practical control problems ranging from autonomous driving~\cite{Saksena2019, Samak2021} to playing video games~\cite{KanervistoHautamaki2020, KanervistoPussinen2020, Vinyals2019}. Despite being tremendously popular due to its simplicity, BC suffers from a range of problems such as distributional shift and causal confusion~\cite{DeHaan2019}. These limitations are addressed using inverse reinforcement learning~\cite{ng2000} and generative adversarial imitation learning~\cite{ho2016generative}, which on the other hand tend to be computationally heavy for complex problems and hard to train.

Recently proposed Video Pre-Training (VPT) model \cite{baker2022video} (see Figure \ref{fig:vpt_architecture}) is a foundation model for BC trained on 70k+ hours of video content scraped from the internet~\cite{baker2022video}. 
VPT is built on an IMPALA \cite{EspeholtKavukcuoglu2018} convolutional neural network (CNN) backbone. The CNN maps an image input to a 1024-dimensional feature vector. VPT generates a batch of 129 vectors and forward them to four transformer blocks. Each block is linked to a memory block containing the last 128 frames. At the end of the transformer pipeline, only the last frame is retained and forwarded to two heads based on Multilayer Perceptrons (MLPs). One head predicts a keyboard action and second head predicts a computer mouse action. 
We provide an analysis of the architecture in Appendix A.





\section{Methods}
Our aim is to solve a complex problem in Minecraft environment, where no explicit reward is available. The only data source that we can utilize is a set of recorded expert trajectories solving that given task. The core idea behind our approach is to reformulate the control problem as a search problem on the experts' demonstrations. 

We use a pre-trained VPT model~\cite{baker2022video} to encode situations in latent space. The pre-trained version of the model used in this study is available at the official GitHub repository~\cite{VPTGithub}. The repository features three foundation models, namely \textit{1x}, \textit{2x} and \textit{3x}. The backbone of the three models is the same, and they differ only for the weights width~\cite{VPTGithub}.



\subsection{Search-based BC}

S-BC solves control problems by retrieving relevant past experiences from experts demonstrations. In this context, we define a \textit{situation} as a set of consecutive observation-action pairs $\{(o_{t}, a_{t}), \dots, (o_{t+n}, a_{t+n})\}$, $n > 0$. 

We illustrate our approach in Figure \ref{fig:approach}. We use VPT to extract all the features embeddings from an arbitrary subset $\mathcal{S}$ of the demonstrations dataset $\mathcal{D}$, $\mathcal{S} \subseteq \mathcal{D}$. The set of these embeddings constitutes the N-dimensional latent space that S-BC searches. Moreover, the expert's optimality assumption~\cite{Russell2019} from IL methods ensures that each situation has been \textbf{addressed} and \textbf{solved} optimally.

During testing, we pass the current situation through VPT. Then, S-BC searches for the most similar embedding point in the space. Here, we compute similarity among any two situations as their L1 distance. We copy the actions of the selected reference situation. At each time-step, we shift the current and reference situations in time and recompute their distance. When situations diverge over time, the approach performs a new \textit{divergence-triggered} search (red lines in Figure \ref{fig:divergence}). If the reference embedding is followed form more than $n$ time-steps, the approach performs a new \textit{time-triggered} search (blue lines in Figure \ref{fig:divergence}).




Our S-BC process is faster than fine-tuning a VPT-based BC agent, training GAIL or RL agent (see Figure \ref{fig:training_time}). At each time-step of the evaluation (Figure \ref{fig:approach}B), the current observation coming from the MineRL environment is encoded through VPT. Then, S-BC compute the L1 distance with the current reference situation. If the two have diverged, a new search in latent space is performed and a new reference situation is selected. Otherwise, we retain the same reference situation. In both cases, S-BC copies the actions coming from the current reference embedding. 


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\columnwidth]{figs/training.pdf}
    \caption{Our approach. (\textbf{A}) \textit{Latent space generation:} trajectories are extracted from the demonstration dataset. Frames are encoded through a provided VPT model, and paired with the corresponding actions. (\textbf{B}) \textit{Evaluation loop:} at each timestep, the new observation is forwarded to the same VPT model. Then, L1 distance across current and reference embeddings is computed and the most similar situation is found. S-BC acts in the environment following the actions of the selected reference situation.}
    \label{fig:approach}
    \vspace{-0.2in}
\end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/training_time.pdf}
    \caption{Time needed to train each agent on 100 trajectories on the FindCave task. In the case of BC models, the training procedure consists of fine-tuning a pre-trained VPT model. For the S-BC model, training means encoding a subset of trajectories through the reference version of VPT. All models have been trained on a single Tesla T4 GPU.}
    \label{fig:training_time}
    \vspace{-0.2in}
\end{figure}

\section{Experiments}
The full FindCave dataset from the MineRL BASALT competition~\cite{ShahDragan2021} consists of 5466 experts' trajectories demonstrating the task, or around 150GB of data. For each frame of an episode, only the unprocessed RGB image and the corresponding action are available. That is, an episode is a set of image-action pairs. No reward signal is available. Similarly, no measure of performance is provided. In our study we use only a small subset of the available data. Specifically, we consider only the first $100$ trajectories.

Additionally, we personally gather expert trajectories for the MineDojo task. For all our tasks, we modified the framework to accept mouse and keyboard inputs and recorded them in the same format as the FindCave dataset. For each task, we record $100$ trajectories. Implementation details about MineDojo modifications and data gathering procedures are reported in Appendix B1.

\subsection{MineDojo tasks}
We compare S-BC against state-of-the-art models in the Minecraft (VPT-based $1x$, $2x$, and $3x$ models) and IRL domains (GAIL). We fine-tune each VPT-based model for two full epochs on our gathered data, and fine-tune a different model for each task. Moreover, we train GAIL using VPT-encoded trajectories, to speed up training by reduce the size of the observation space. We train GAIL for ~6h for each task. We evaluate the models in two ways. First, we use the MineDojo \cite{fan2022minedojo} framework to provide clear numerical results. 

In the suite, authors distinguish \textit{ground-truth} and \textit{creative} tasks. On one hand, ground-truth tasks feature a well-defined terminal condition, such as "kill a specific unit" or "gather $x$ quantity of material", and are separates in broad categories such as \textit{combat}, \textit{build}, \textit{harvest}, and so on. On the other hand, creative tasks do not feature a terminal condition. Although, they can be evaluated indirectly through MineCLIP \cite{fan2022minedojo} by mapping a text prompt and a video frame in a shared latent space and then computing cosine distance to assess similarity between them. Such similarity score is computed for each timestep, as in standard RL. 

For our experiments, we select four ground-truth tasks, namely, \textbf{combat spider} and \textbf{combat zombie} from the \textit{combat} category and \textbf{harvest log}, \textbf{harvest wheat seed} from the \textit{harvest} category, and two \textit{creative} tasks, \textbf{"find ocean"} and \textbf{"dig a hole"}. 

\subsection{FindCave}
As second set of experiments, we compare the agents directly on the FindCave task from BASALT \cite{Milani2023}, where no reward information is known or obtainable. To support the evaluation process, we train a simple binary classifier to detect the presence of a cave. Our classifier is composed by four convolutional layers and two fully-connected layers. The network has been trained with supervised learning on a dataset of cave frames, extracted from the original FindCave data, and achieved a validation accuracy of $97.89\%$ over it. Further details are discussed in Appendix B2. To ensure fairness over the amount of accessible relevant knowledge to each model, we use the same subset of $100$ trajectories from the original BASALT dataset on them.

We apply minimal changes to the task rules with respect to the official competition, to ease the evaluation procedure while keeping the performance evaluation intact. First, we disable the terminal action \textit{'ESC'} in all the agents. We support this decision by highlighting that terminal actions constitute a minimal fraction of the amount of training data, and a BC agent would likely ignore it, or use it incorrectly. Therefore, we removed the action to evaluate the Second, the BASALT competition considers an episode successful whenever an agent performs the terminal action while being inside a cave. Instead, we consider an episode successful whenever an agent spends more than five seconds in a cave. The maximum time limit for each evaluation episode is set to three minutes, similarly to the official competition rules.

As in the evaluation process of the BASALT competition, we test our agent on twenty seed values. Since the official values used in BASALT evaluation are not publicly available, we have selected each seed manually to ensure the presence of caves. For each run, we play 10 evaluation episodes.

\paragraph{Latent space visualization}
We perform a study over the latent space used from our agent. We plot t-SNE representation of a full latent space and evaluate position of the cave frames, similarity between close points. Finally, we track the movement of an agent using such latent space, to study its dynamics.


\paragraph{Evaluation procedure}
Our evaluation procedure is as follows. First, we let an agent play the evaluation episodes and record each one of them. Then, we pass each frame of the video to the classifier, and label them as either \textit{cave} or \textit{non-cave} frames. Whenever a cave frame is detected, we start counting the number of consecutive cave frames. Following the MineRL specification \cite{GussSalakhutdinov2019}, we assign each frame a duration of $0.05$s. This lead to set the threshold of five seconds to $100$ consecutive cave frames. Whenever such threshold is exceeded, we consider an episode successful.

To account for unique situations, we run additional evaluations lowering the time threshold. For each spotted situation, we take a look at the current frame and evaluate it manually. Unique situations include, but are not limited to, agent reaching a cave and being killed before the five second mark, agent digging a cave itself (not allowed from BASALT competition rules), or agent walking in exceptionally dark areas that might be mistaken as caves.

\section{Results}

\begin{table*}
\centering
{\addtolength{\tabcolsep}{0pt}
\begin{tabular}{c c c c c c}
  & \textbf{BC 1x} & \textbf{BC 2x}  & \textbf{BC 3x} & \textbf{GAIL} & \textbf{S-BC (Ours)} \\[2pt] \hline \\[-7pt]
Find Ocean & $20.25\pm1.10$ & $20.19\pm1.04$ & $19.82\pm1.05$ & $20.30\pm0.74$ & $\textbf{20.47}\pm1.11$\\[2pt] \hline \\[-7pt]
Dig Hole                               & $20.80\pm0.88$                              & $20.94\pm0.85$     & $20.95\pm0.87$ & 
$20.20\pm0.24$ &  $\textbf{20.97}\pm0.92$                               \\[2pt] %
\end{tabular}
\caption{Average MineCLIP score and its standard deviation per model on the evaluated \textit{creative} tasks. MineCLIP scores can be used to train agents in the MineDojo suite in an RL fashion.}
}
\label{tab:mineclipscores}
\end{table*}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/dojo_results.pdf}
    \vspace{-0.1in}
    \caption{Results for six MineDojo tasks. \textbf{(A)} Model success rate over 100 evaluation episodes. Reference baseline model BC 1x is highlighted with a horizontal blue line in each plot. \textbf{(B)} Average completion time for each task. Tasks that have never been completed are associated with a blank space. Tasks completed only one time show a single line corresponding to the completion time of that single success.}
    \label{fig:dojo_results}
    \vspace{-0.2in}
\end{figure}

\subsection{MineDojo tasks}

We evaluate our models over six diverse tasks of the MineDojo suite. Figure \ref{fig:dojo_results} shows the models success rate and completion time for each task. Additionally, we report in Table \ref{tab:mineclipscores} the average score obtained by each model in each creative task.

Notably, S-BC performs similarly or better than its competitors. Figure \ref{fig:dojo_results}A shows that our method is the only one able to complete instances of the combat tasks. In harvest tasks, our model either performs similarly or lose a mere 5\% in performance with respect to much bigger, learning-based models. It is also interesting to notice that VPT-based foundation model were originally trained on the ObtainDiamond track~\cite{kanervisto2022minerl}, which first step consists in collecting logs. We highlight that GAIL was not able to complete any of the ground-truth tasks. We point out that we have trained GAIL for a time that is comparable to the fine-tuning time of the VPT-based models (~1h). Therefore, due to the limited amount of time used for training, it might under perform on some tasks.

Figure \ref{fig:dojo_results}B shows the average time of completion for successful episodes. We highlight that S-BC requires either the same on less time to complete, on average. Our agent is on average the faster in completing \textbf{harvest one log}, and performs similarly in \textbf{harvest one wheat seed}. In the \textbf{combat spider} case, S-BC was the only method able to complete the task consistently, using on average two thirds of the time at its disposal.

Table \ref{tab:mineclipscores} describes the results of the \textbf{creative} tasks. According to MineCLIP, all the models performed similarly. It is interesting to notice that in creative tasks, GAIL seems to achieve comparable performance to other methods.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/comparison.pdf}
    \caption{Average success rate for our tested model on the FindCave task over $3$ runs. Each agent has been evaluated over $20$ seeds, playing 10 episodes on each seed. Baseline model is highlithed with a vertival blue line.}
    \label{fig:cave_results}
    \vspace{-0.2in}
\end{figure*}

\subsection{FindCave}
We report success rate for the models on the FindCave task in Figure \ref{fig:cave_results}. S-BC has obtained the best performance, being able to complete the task 40\% of the times. GAIL was never able to find a cave, while VPT-based BC models were quite successful, reporting success rates of $15\%$, $25\%$ and $30\%$ for the \textit{1x}, \textit{2x}, and \textit{3x}. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=0.95\textwidth]{figs/latent_plots.pdf}
    \caption{t-SNE diagrams of S-BC latent space with $10$ trajectories. \textbf{(A)} Separation between exploration (blue) and cave (red) frames. Some examples of cave frames are linked to the corresponding point (symbols) in the latent space. \textbf{(B)} t-SNE representation of the same space with points separated according to their belonging trajectory. Cave frames for each trajectory are marked with a matching color star symbol. \textit{Zoom:} a close-up look at some clustered cave frames coming from different trajectories.}
    \label{fig:latent_plot}
    \vspace{-0.2in}
\end{figure*}

\subsection{Latent space visualization}
We have analyzed the VPT latent space used by our models and its transformation over the number of encoded trajectories. To visualized it, we have used t-SNE \cite{hinton2008} plotting. Figures~\ref{fig:latent_plot}A and~\ref{fig:used_trajectories} show two examples of latent space used by S-BC, with $10$ and $25$ encoded trajectories respectively. We have classified each point as either a cave (red) or exploration frame (blue). We used our cave classifier to determine all cave frames. In our study, we have analyzed visual hints of structure of those spaces. Additionally, we have extracted some meaningful pieces of information such as similarity across frames and the search path of an episode.

\subsubsection{Space structure \& cave frames}
Both $10$ and $25$ trajectories latent space plots (Figure \ref{fig:latent_plot}A and \ref{fig:used_trajectories}, respectively) show that the embeddings in the VPT latent space can be separated to some degree, but are quite dense. Perhaps not surprisingly, an increase in the number of encoded trajectories results in a less structured space. This is supported by the visual appearance of a Minecraft frame: the game features several biomes, that range from desert to snowy mountains. In the FindCave task, an agent is bounded to spawn in a plain biome. Such biome is characterized by the presence of fields, forests, ponds and, sometimes, lakes or sea. Therefore, a number of visually different frames are possible. But, whenever switching from two different environments (e.g. from lake to forest), we expect some "transition frames" that contain a mixture of elements of both. In a visualization method such as t-SNE, we expect such frames to be equally distant from proper examples of any of the two environments. That is, we expect them to be in the middle of two more dense regions of space. So, as the number of trajectories increase, we might expect the number of transition frames to increase, thus making well-defined clusters more rare.

The position of cave frames within the space constitute another notable result of this visualization. The vast majority of cave frames are grouped in half of the space. Within this region, some clusters are easily spotted, but in general cave frames tend to be sparse.

\subsubsection{Visual similarity across points}
In our study, we have visualized several frames of the latent space, to understand the relation between their visual resemblance and spatial coordinates. We show some examples in Figure~\ref{fig:latent_plot}A: frames linked with a \textit{green} symbol are cave frames belonging to the same trajectory; frames corresponding to an \textit{orange} symbol are cave frames coming from different trajectories; finally, frames marked with a yellow symbol are exploration frames belonging to the same cluster. 

By comparing green and orange examples, it is clear that each cave cluster contains frames from a different trajectory. Additionally, frames linked to a yellow symbol show how each cluster is formed by visually similar examples. Such morphology of the space suggests that, depending on the current situation, an S-BC agent will select a close point whenever the visual transition across situations is smooth. On the contrary, whenever the observation drastically changes, the agent will look for a distant new situation to follow. 

To account for the points distribution of each trajectory, we have plotted a second version of the $10$ trajectories latent space (Figure \ref{fig:latent_plot}B). In this representation, each point is colored according to its belonging trajectory. We have marked the cave frames of a specific trajectory with a star symbol of the same color. 

Notably, each cluster contains points of a variety of colors. This supports the fact that visual resemblance plays a fundamental role in deciding a point position within the space: similar frames (e.g. fields, forests, and so on) coming from different trajectories are squeezed together. Therefore, one might conclude that VPT embeddings are heavily biased towards visual similarity. While we believe that such metric is indeed important, we have identified clues that suggest other important factors in defining them. In particular, we believe that past information is another key factor in this regard. To support this claim, consider the yellow examples: while the square and triangle seems to be the most visually similar pair, their distance is greater than e.g. triangle and rhombus. Such observation imposes to consider other factors in the characterization of a VPT embedding.

\subsubsection{Example of one episode using S-BC}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.5\columnwidth]{figs/used_trajectories.pdf}
    \caption{Visualization of the VPT embeddings latent space with 25 trajectories encoded. A yellow point marks a trajectory used from the agent during the corresponding episode.}
    \label{fig:used_trajectories}
    \vspace{-0.2in}
\end{figure}
We have visualized the situations that an S-BC agent trained on 25 trajectories has followed in a successful evaluation episode. The result is shown in Figure~\ref{fig:used_trajectories}. Each yellow dot corresponds to a new search performed by our agent at some point in the episode. Notably, $4$ out of $6$ searches were performed in a cave frames cluster. In the episode, the agent enters the cave after around $15$s. Then, it wanders there and gets killed after $30$s. The fact that our agent has performed a total of $6$ searches suggests that, on average, it has followed each selected trajectory for $5$s (around $100$ frames).

\subsection{Perceptual evaluation}

\begin{table*}[!t]
\centering
{\begin{tabular}{c c c c c c}
\hline \\[-6pt]
\textbf{Team} & FindCave & MakeWaterfall & AnimalPen & House & \textbf{Average} \\[1pt]
 \hline \\[-6pt]
GoUp & $0.31$ & $\textbf{1.21}$ & \textbf{0.28} & \textbf{1.11} & \textbf{0.73} \\[1pt]
\textbf{Our approach} & \textbf{0.56} & -0.10 & 0.02 & 0.04 & \textbf{0.13} \\ [1pt]
voggite & 0.21 & 0.43 & -0.20 & -0.18 & \textbf{0.06} \\[1pt]
JustATry & -0.31 & -0.02 & -0.15 & -0.14 & \textbf{-0.15} \\[1pt]
TheRealMiners & 0.07 & -0.03 & -0.28 & -0.38 & \textbf{-0.16} \\[1pt]
\hline \\[-6pt]
Human2 & 2.52 & 2.42 & 2.46 & 2.34 & \textbf{2.43} \\[1pt]
Human1 & 1.94 & 1.94 & 2.52 & 2.28 & \textbf{2.17} \\[1pt] \hline \\[-6pt]
BC-Baseline & -0.43 & -0.23 & -0.19 & -0.42 & \textbf{-0.32} \\[1pt]
Random & -1.80 & -1.29 & -1.14 & -1.16 & \textbf{-1.35} \\[1pt] \hline \\[-9pt]
\end{tabular}
\caption{Top-5 ranking of the NeurIPS BASALT 2022 competition~\protect\cite{Milani2023}. Below, the TrueSkill~\protect\cite{minka2018trueskill} scores for two human expert players, a BC baseline and a random agent are reported for comparison.}
}
\label{tab:results}
\vspace{-0.2in}
\end{table*}

To determine its rank among the participants, the organizers of the competition have used the TrueSkill~\cite{minka2018trueskill} ranking system, which is widely used in the Microsoft online gaming ecosystem. Given a set of competitors, the system uses Bayesian inference to compute an ELO-like score, according to the match history of each competitor.

In the context of the BASALT competition, the system considers each trained agent as a participant. To create a match history for each of them, any two participants are drawn and their evaluation videos are judged by a human contractor. For each pair of videos, the contractor indicates which agent was able to solve the task (or which one was closer), and how human-like an agent appeared to be. Those two ratings are then aggregated to the match history of each competitor. When a suitable amount of outcomes are available for an agent, the TrueSkill for that agent is computed.

Our proposed S-BC agent was overall ranked second place in the challenge. The results of our agent are described in \ref{tab:results}. First place was awarded to team GoUp. Their method uses detection methods and leverages human knowledge of the task through scripting \cite{Milani2023}. Notably, all the other learning-based methods achieved lower performance than S-BC. Additionally, our method was awarded with $2$ out of $5$ research innovation prizes.

\subsubsection{Behavior of agents in videos}
In our study we have collected and analyzed a wide number of videos that demonstrate the general behavior of each agent. From those, we were able to delineate some differences in the behavior of BC and S-BC agents:
\paragraph{BC models}
As a premise, it is important to note that the reference version of VPT provided by the organizers of the competition was trained on data from the MineRL ObtainDiamond track~\cite{kanervisto2022minerl} and then fine-tuned on the BASALT~\cite{ShahDragan2021, Milani2023} dataset. Judging from the videos, our additional fine-tuning towards the FindCave task shows some improvements of the agents. Overall, though, the general behavior remains the primary objective of the ObtainDiamond competition: it is not rare that a BC agent chops trees as first step. We believe that the limited amount of episodes used for fine-tuning has had a clear negative impact on the performance. We expect an agent fine-tuned on the full FindCave dataset to be more aligned with the expected FindCave behavior, at the cost of a drastic increase in training time.
\paragraph{S-BC}
We found our agent to be quite robust in performance, and be human-like at the same time. S-BC shows significantly more aligned behavior with the proposed task than any BC agent. In general, our agent is able to recover meaningful trajectories when the cave is nearby. Despite this, our agent is far from being perfect: in some instances, S-BC has shown dichotomic behavior regarding caves. At first, the agent would face a cave and quickly turn around. In the following seconds, a new search correctly guiding the agent towards the same cave was performed. We believe that this behavior comes from the possible presence of enemies in caves, which would influence the retrieval of a better suited reference situation.

\section{Conclusions}
We introduced S-BC, a BC-inspired search-based approach that uses the past experience of experts to solve similar control problems. Our approach shows better or similar performance, requiring less training time, allowing a few-shot learning, and multi-skill performance when skill demonstration is provided. We applied our method to the MineRL BASALT NeurIPS 2022 Challenge, where our agent reached overall 2nd place. 
The agent had to demonstrate human-like behavior while completing the tasks. Numerical evaluations over a suite of MineDojo tasks shows that our agent reaches similar or better performance than state-of-the-art BC and IRL methods, while requiring no re-training or fine-tuning.



\bibliography{bibliography.bib}
\bibliographystyle{ieeetr}

\newpage
